What makes multilingual BERT multilingual?

Recently, multilingual BERT works remarkably well on cross-lingual transfer tasks, superior to static non-contextualized word embeddings. In this work, we provide an in-depth experimental study to supplement the existing literature of cross-lingual ability. We compare the cross-lingual ability of non-contextualized and contextualized representation model with the same data. We found that datasize and context window size are crucial factors to the transferability.

==> sections/alignment_old.tex <==
\section{How to Build up Cross-lingual Ability}
\label{section:align}
Cross-lingual alignment of words in m-BERT representation has been observed and credited with cross-lingual transferability~\citep{Cao:20}. The transferbility come from semantically similar words are encoded into similar latent representations, regardless of languages. Considering  that m-BERT was trained on masked language modeling and there are a bunch of subwords shared by languages that could be used as anchors, it is hypothesized that m-BERT exploited the co-occurrence information to align word pairs having similar contexts or usage statistics~\citep{pires2019multilingual}. 

However, m-BERT seems to be the only model succeeding in aligning cross-lingual word pairs simply trained on concatenated monolingual corpora with a monolingual objective. Similar methods for training cross-lingual word embeddings, called unsupervised joint training, often fail to generate high-quality alignments, especially for embeddings of non-shared words, due to a lack of explicit clues~\citep{Wang:20}. \citet{Wang:20} show that supervised post-hoc alignment effectively boosts unsupervised joint training in the case of traditional non-contextualized embeddings, but is not as beneficial in the case of m-BERT, suggesting that pretraining alone generates strong alignments even without supervision. %Lee: 這個敘述應該要引用論文
%Liang: 我先cite一篇 但他有點進步 我不確定宗嫄是看到哪一篇
%T: 其實是同一篇(Wang:20)裡有講，我寫的不太好，我就一起補上去了

Several key components have been studied why m-BERT generalize across languages so well~\citep{Karth:20}. In an analysis of the two-language version of BERT, it was shown that depth and the total number of network parameters affect cross-lingual ability a lot. Performance on the XNLI dataset significantly degrades when model architecture becomes shallower or more-parsimonious. Wordpiece tokenization also contributes to cross-lingual ability, compared with character-level or word-level tokenization. 

Surprisingly, shared vocabulary was found to be unnecessary in the same study. Pre-trained BERT successfully transfers from English to a lexical-modified version of English, although it failed when word ordering or n-gram statistics were randomly manipulated. This suggests that some structural similarity is possibly what BERT has learned from, while further definition should be developed and discovered. 

It's also unclear if the above findings hold for other non-contextualized embedding models, since the pre-training process and dataset could make a crucial difference in cross-lingual ability. %%T:這句感覺有更informative的寫法
%In this section, we want to answer some comparative questions orthogonal to previous literature, which was studied either in the scope of BERT itself or between different embedding methods but didn't normalize the effect of pre-training data. We would like to find out if trained under same corpus and tokenization, will BERT still have overwhelming advantage over other traditional non-contextualized methods?   

In this section, we calibrate the external factors when pretraining the representations to give a fair discussion focusing on the architecture of the embedding models and study two key components that are dominant in building up cross-lingual ability of m-BERT.  

\subsection{Metrics for Cross-lingual Ability}
There are two main paradigms for evaluating cross-lingual representations:~{\it word retrieval} and {\it downstream task transfer}. 
Here we use both word retrieval and downstream task transfer as the indicators of cross-lingual ability for both contextualized and non-contextualized embeddings. 
Although word retrieval is a task originally proposed to measure cross-lingual alignment at the word level, therefore naturally more suitable for non-contextualized embeddings, contextual version of word retrieval has been proposed for contextualized embeddings and consistent with downstream task transfer performance~\citep{Cao:20}. 

\subsubsection{Word Retrieval}
Given a word and a bilingual dictionary~$D=\{(x_1,y_1),(x_2,y_2),\ldots,(x_n,y_n)\}$, listing all parallel word pairs from source and target languages, word retrieval is the task to retrieve the corresponding word in target language considering information provided by embedding vectors~$\{(u_1,v_1),(u_2,v_2),...(u_n,v_n)\}$. Specifically we consider a nearest neighbor retrieval function
\begin{equation}
    \text{neighbor}(i)=\mathop{\arg\max}_{j}\text{sim}(u_i,v_j),
\end{equation}
where $u_i$ is the embedding of source word $x_i$ and we want to find its counterpart $y_i$ among all candidates~$y_1,y_2,...y_n$. And we use cosine similarity as the similarity function $\text{sim}$ .
%\begin{equation}
%sim(u_i,v_j) = \frac{u_i \cdot v_i}{|u_i||v_i|}.%T:誰來救救我的norm symbol
%\end{equation}

Then we have{\it~mean reciprocal rank }(MRR) as evaluation metrics. MRR is defined as
\begin{equation}
\text{mean reciprocal rank} = \frac{1}{n}\sum_{i}^{n}\frac{1}{\text{rank}(y_i)}
\end{equation}
where $\text{rank}(y_i)$ is a ranking function based on retrieval results.
For contextualized embeddings, we simply average embeddings in all contexts and use the mean vector to represent each word, so that contextualized embeddings could also be evaluated with the task defined above.

%\subsubsection{Zero-shot Transfer XNLI}
\subsubsection{Downstream Task Transfer}
We consider XNLI as our downstream task to evaluate cross-lingual transfer. The XNLI dataset was constructed from the English MultiNLI dataset by keeping the original training set but human-translating development and test sets into other 14 languages~\citep{conneau:18, williams:18}. Given a pair of sentences, the task is to predict the relation of the sentence pair among three classes: entailment, neutral, or contradiction. As there are only training data in English, models should perform zero-shot cross-lingual transfer on development and test sets.

\subsection{Experiments}
To compare non-contextualized and contextualized embedding models, we conducted experiments with GloVe, Word2Vec and, BERT, where the number of dimensions was all set to 768. Embeddings were first pretrained from scratch and then evaluated on word retrieval and XNLI, to assess their cross-lingual ability.   

For pretraining data, we used Wikipedia from 15 languages~(English, French, Spanish, German, Greek, Bulgarian, Russian, Turkish, Arabic, Vietnamese, Thai, Chinese, Hindi, Swahili, and Urdu) to pre-train all word embeddings following unsupervised joint training scenario, assuring each target language in the downstream task has been well pre-trained. 

For word retrieval task, we evaluated cross-lingual alignment between English and each of the remaining 14 languages, using bilingual dictionaries from MUSE\footnote{https://github.com/facebookresearch/MUSE}.
For XNLI zero-shot transfer task, the training set is in English, and the target languages of testing sets are the same as those used in the word retrieval task.  

To eliminate the effect of tokenization, we tokenized data uniformly with the vocabulary of m-BERT, especially the cased one, which is essentially wordpiece tokenization. 

Also, we experimented with different amounts of data: {\it 200k} and {\it 1000k} sentences per language to study the results under different data sizes. 
The results with {\it 200k} and {\it 1000k} sentences are shown in Sections~\ref{subsubsection:small} and~\ref{subsubsection:big}, respectively.  

\subsubsection{Small Pretraining Data}
\label{subsubsection:small}
\begin{figure}[t!]
\centering 
\includegraphics[width=\linewidth]{sections/figs/mrr_small.pdf}
 \caption{Evaluating alignment with Word Retrieval, compared between different representation models. For reference, Google BERT is the m-BERT pre-trained by Google. Except for Google Bert, other embeddings were pre-trained on the same data (200k sentences per language).}
 \label{fig:3_1}
 \vspace{-0.25cm}
\end{figure}
Surprisingly, when pre-trained on small pretraining data (200k sentences per language), BERT didn't show its extraordinary cross-lingual ability as shown in Figure~\ref{fig:3_1} and \ref{fig:3_2}. For example, GloVe and Word2Vec achieved stronger cross-lingual alignment than BERT in terms of MRR score on word retrieval task on every language paired with English. And although BERT achieved better accuracies on XNLI zero-shot transfer on several languages, the margins were very small, and the overall performances were not better than GloVe and Word2Vec.  

This finding provides a further discussion of the literature. Work by ~\citet{Karth:20} has found that depth and the total number of network parameters were two decisive architecture elements dominating the cross-lingual ability of BERT, also supported by experiments on XNLI. 
When the number of attention heads and the number of total parameters were fixed, decreasing model depth degenerated cross-lingual transfer performance. On the other hand, when the number of attention heads and depth were fixed, decreasing the number of network parameters degenerated performance, either. 
It seems that the expressiveness or capacity of models is crucial to building up cross-lingual ability. 

However, is it really the case that the bigger, the better? 
From results in this experiment, the capacity of BERT is definitely much bigger than GloVe and Word2Vec, but in the case of pretraining on the limited size of data, BERT didn't achieve superior performance as expected, suggesting that the relation of model capacity and cross-lingual ability may not be monotonic and the size of pretraining data also comes into play. 

\begin{figure}[t!]
\centering 
\includegraphics[width=\linewidth]{sections/figs/XNLI_small.pdf}
 \caption{Performance comparison on XNLI zero-shot cross-lingual transfer task}
 \label{fig:3_2}
\end{figure}
\vspace{-0.25cm}
\subsubsection{Big Pretraining Data}
\label{subsubsection:big}
\begin{figure}[t!]
\centering 
\includegraphics[width=\linewidth]{sections/figs/mrr_big.pdf}
 \caption{Evaluating alignment with Word Retrieval, compared between different representation models. For reference, Google BERT is the m-BERT pre-trained by Google. Except for Google BERT, other embeddings were pre-trained on the same data (1000k sentences per language).}
 \label{fig:3_3}
 \vspace{-0.25cm}
\end{figure}
When pre-trained on big pretraining data (1000k sentences per language), there was a dramatic turn as shown in Figure~\ref{fig:3_3} and~\ref{fig:3_4}. BERT achieved an overwhelmingly higher MRR score than other embeddings on every XX-En language pairs, showing that it did a much better job in aligning semantically similar words from different languages. 

Testing results on XNLI were also consistent with word retrieval task, BERT reached higher accuracies than GloVe and Word2Vec, demonstrating that it had the better cross-lingual ability.  

It was noticeable that the increase in pretraining data size largely improved the cross-lingual alignment and transferability of BERT, while it was not the same case for GloVe and BERT. And the bounding performance of Google BERT, which is the pretrained parameters released by Google, shows that there is still room for improvement if given even more pretraining data.

Besides the effect of amount of data, in the next subsection, we further studied other key components making BERT capable of learning a good cross-lingual representation space.
\begin{figure}[t!]
\centering 
\includegraphics[width=\linewidth]{sections/figs/XNLI_big.pdf}
 \caption{Performance comparison on XNLI zero-shot cross-lingual transfer task}
 \label{fig:3_4}
 \vspace{-0.25cm}
\end{figure}

\subsubsection{Breaking Down Long Dependency}
We noticed that the typical co-occurrence window size of non-contextualized embeddings, like GloVe and Word2Vec,  are often limited to 5$\sim$30 tokens, but BERT could attend to hundreds of tokens, which means that BERT could learn from longer dependency and richer co-occurrence statistics. So we experimented with a smaller window size to find out if longer dependency is also necessary for learning cross-lingual structures.    
We directly sliced sentences in original pretraining data into smaller segments, limiting input length to 20 tokens for each example. And then we evaluated embeddings pretrained on these segments for cross-lingual ability\footnote{Limiting the number of tokens attended by attention heads may not work because the information from far tokens could still flow through layers and be collected at deeper layers.}.   


\begin{figure}[t!]
\begin{subfigure}{\linewidth}
  \includegraphics[clip,width=\linewidth]{sections/figs/windowsize_200.pdf}%
\end{subfigure}
\begin{subfigure}{\linewidth}
  \includegraphics[clip,width=\linewidth]{sections/figs/windowsize_1000.pdf}%
\end{subfigure}
\caption{The Effect of Window Size}
\label{fig:3_5}
\vspace{-0.25cm}
\end{figure}

Results are shown as figure~\ref{fig:3_5}. In the case of big pretraining data, pretraining BERT with shortened inputs drastically hurt the cross-lingual ability of BERT, indicated by lower MRR score on word retrieval task compared to BERT pre-trained on normal-lengthed data. It should be noticed that the total number of tokens in pretraining data stayed unchanged.

However, in the case of small pretraining data, pretraining BERT with shortened inputs yielded to better cross-lingual alignment on several languages, suggesting that breaking down long dependency helps BERT to learn better cross-lingual alignment when only limited data is available.  

In Figure~\ref{fig:3_6},  it is shown that when there were no long dependencies to learn, the benefit of increasing the datasize became minor. 
The results on XNLI also show that breaking down long dependency was more harmful when there were more pretraining data.   

\begin{figure}[t!]

\begin{subfigure}[b]{\linewidth}
  \includegraphics[clip,width=\linewidth]{sections/figs/windowsize_xnli_all.pdf}
  \subcaption{When limiting context window, the effect of pretraining datasize is less significant on XNLI transfer performance}
\end{subfigure}

\begin{subfigure}[b]{\linewidth}
  \includegraphics[clip,width=\linewidth]{sections/figs/windowsize_xnli_decrease_per.pdf}
  \subcaption{Performance drop on XNLI due to limiting context window size (original 512$\rightarrow$20) is shown in percentage. It is shown that the performance decrease of BERT pre-trained on small data is less than big data and even negative on some languages, which means there is an increase in transfer}
\end{subfigure}
\caption{The Effect of Window Size}
\label{fig:3_6}
\vspace{-0.25cm}
\end{figure}

\begin{figure}[t!]
\centering 
\includegraphics[width=\linewidth]{sections/figs/Word2Vec (1).pdf}
 \caption{The Effect of Window Size on Word2Vec}
 \label{fig:3_7}
 \vspace{-0.25cm}
\end{figure}
We further checked the case of Word2Vec, varyring window size to 128 and 256 on small pretraining data. The alignment evaluation via MRR is shown in Figure~\ref{fig:3_7}. On most of the languages, increasing window size to 128 improved cross-lingual alignment on Word2Vec embeddings. However, increasing window size to 256 was not as beneficial, suggesting there may be a bottleneck from model capacity.

Considering the above observations, we hypothesized that cross-lingual alignment or cross-lingual transferability of BERT are learned not only from local co-occurrence relations but also from co-occurrence relations of global scope, with a larger amount of data and model capacity required.

\subsubsection{Word Retrieval Part-of-speech Analysis}
At last, to gain insight into where alignment happens and which type of tokens are aligned best in our pretrained BERT (1000k), we analyzed the MRR score by part-of-speech tag obtained from the OntoNotes Release 5.0~\footnote{https://catalog.ldc.upenn.edu/LDC2013T19}dataset. We simply associated each token in m-BERT vocabulary with its most common part-of-speech label from OntoNotes annotations and calculated MRR for each class of part-of-speech tag. For simple comparison, we further grouped all the part-of-speech tags into closed-class and open-class two classes, as shown in table~\ref{tab:mrr_by_pos}, where fixed sets of words serving grammatical functions fall into closed-class and lexical words (e.g. noun, verb, adjective and adverb) fall into open-class. Different from \citet{Cao2020Multilingual}'s work, we showed that our BERT has higher alignment score for open-class versus closed-class categories. And among open-class of part-of-speech tags, adjectives are better aligned, on top of nouns, adverbs and verbs.        

\input{sections/tables/mrr_by_label}

==> sections/alignment_old_v2.tex <==
\section{How to Build up Cross-lingual Ability}
\label{section:align}

%Cross-lingual alignment of words in m-BERT representation has been observed and credited with cross-lingual transferability~\citep{Cao:20}. The transferbility come from semantically similar words are encoded into similar latent representations, regardless of languages. Considering  that m-BERT was trained on masked language modeling and there are a bunch of subwords shared by languages that could be used as anchors, it is hypothesized that m-BERT exploited the co-occurrence information to align word pairs having similar contexts or usage statistics~\citep{pires2019multilingual}. 

%However, m-BERT seems to be the only model succeeding in aligning cross-lingual word pairs simply trained on concatenated monolingual corpora with a monolingual objective. 
%Similar methods for training cross-lingual word embeddings, called unsupervised joint training, often fail to generate high-quality alignments, especially for embeddings of non-shared words, due to a lack of explicit clues~\citep{Wang:20}. 
%\citet{Wang:20} show that supervised post-hoc alignment effectively boosts unsupervised joint training in the case of traditional non-contextualized embeddings, but is not as beneficial in the case of m-BERT, suggesting that pretraining alone generates strong alignments even without supervision. %Lee: 這個敘述應該要引用論文
%Liang: 我先cite一篇 但他有點進步 我不確定宗嫄是看到哪一篇
%T: 其實是同一篇(Wang:20)裡有講，我寫的不太好，我就一起補上去了

%Several key components have been studied why m-BERT generalize across languages so well~\citep{Karth:20}. In an analysis of the two-language version of BERT, it was shown that depth and the total number of network parameters affect cross-lingual ability a lot. Performance on the XNLI dataset significantly degrades when model architecture becomes shallower or more-parsimonious. Wordpiece tokenization also contributes to cross-lingual ability, compared with character-level or word-level tokenization. 

%Surprisingly, shared vocabulary was found to be unnecessary in the same study. Pre-trained BERT successfully transfers from English to a lexical-modified version of English, although it failed when word ordering or n-gram statistics were randomly manipulated. This suggests that some structural similarity is possibly what BERT has learned from, while further definition should be developed and discovered. 

%It's also unclear if the above findings hold for other non-contextualized embedding models, since the pre-training process and dataset could make a crucial difference in cross-lingual ability. %%T:這句感覺有更informative的寫法

%In this section, we want to answer some comparative questions orthogonal to previous literature, which was studied either in the scope of BERT itself or between different embedding methods but didn't normalize the effect of pre-training data. We would like to find out if trained under same corpus and tokenization, will BERT still have overwhelming advantage over other traditional non-contextualized methods?   

%In this section, we calibrate the external factors when pretraining the representations to give a fair discussion focusing on the architecture of the embedding models and study two key components that are dominant in building up cross-lingual ability of m-BERT.  

\subsection{Metrics for Cross-lingual Ability}
There are two main paradigms for evaluating cross-lingual representations:~{\it word retrieval} and {\it downstream task transfer}. 
Here we use both as the indicators of cross-lingual ability.
Although word retrieval is a task originally proposed to measure cross-lingual alignment at the word level, therefore naturally more suitable for non-contextualized embeddings, contextual version of word retrieval has been proposed for contextualized embeddings and consistent with downstream task transfer performance~\citep{Cao:20}. 

\subsubsection{Word Retrieval}
Given a word and a bilingual dictionary~$D=\{(x_1,y_1),(x_2,y_2),\ldots,(x_n,y_n)\}$, listing all parallel word pairs from source and target languages, word retrieval is the task to retrieve the corresponding word in target language considering information provided by embedding vectors~$\{(u_1,v_1),(u_2,v_2),...(u_n,v_n)\}$. Specifically we consider a nearest neighbor retrieval function
\begin{equation}
    \text{neighbor}(i)=\mathop{\arg\max}_{j}\text{sim}(u_i,v_j),
\end{equation}
where $u_i$ is the embedding of source word $x_i$ and we want to find its counterpart $y_i$ among all candidates~$y_1,y_2,...y_n$. 
We use cosine similarity as the similarity function $\text{sim}$.

%\begin{equation}
%sim(u_i,v_j) = \frac{u_i \cdot v_i}{|u_i||v_i|}.%T:誰來救救我的norm symbol
%\end{equation}

Then we have{\it~mean reciprocal rank }(MRR) as evaluation metrics. 
\begin{equation}
\text{MRR} = \frac{1}{n}\sum_{i}^{n}\frac{1}{\text{rank}(y_i)}
\end{equation}
where $\text{rank}(y_i)$ is a ranking function based on retrieval results.
For contextualized embeddings, we average embeddings in all contexts and use the mean vector to represent each word, so that contextualized embeddings could also be evaluated with the task defined above.

%\subsubsection{Zero-shot Transfer XNLI}
\subsubsection{Downstream Task Transfer}
We consider XNLI as our downstream task to evaluate cross-lingual transfer. The XNLI dataset was constructed from the English MultiNLI dataset by keeping the original training set but human-translating development and test sets into other 14 languages~\citep{conneau:18, williams:18}. 
%Given a pair of sentences, the task is to predict the relation of the sentence pair among three classes: entailment, neutral, or contradiction. 
As there are only training data in English, models should perform zero-shot cross-lingual transfer on development and test sets.

\subsection{Experimental Setup}
To compare non-contextualized and contextualized embedding models, we conducted experiments with GloVe, Word2Vec and, BERT, where the number of dimensions was all set to 768. 
To eliminate the effect of tokenization, we tokenized data uniformly with the vocabulary of m-BERT, especially the cased one, which is essentially wordpiece tokenization. 
Embeddings were first pretrained from scratch and then evaluated on word retrieval and XNLI, to assess their cross-lingual ability.   
For pretraining data, we used Wikipedia from 15 languages~(English, French, Spanish, German, Greek, Bulgarian, Russian, Turkish, Arabic, Vietnamese, Thai, Chinese, Hindi, Swahili, and Urdu) to pre-train all word embeddings following unsupervised joint training scenario, assuring each target language in the downstream task has been well pre-trained. 

For word retrieval task, we evaluated cross-lingual alignment between English and each of the remaining 14 languages, using bilingual dictionaries from MUSE\footnote{https://github.com/facebookresearch/MUSE}.
For XNLI zero-shot transfer task, the training set is in English, and the target languages of testing sets are the same as those used in the word retrieval task.  

\subsection{Small Pretraining Data}
\label{subsubsection:small}

We experimented with different amounts of data: {\it 200k} and {\it 1000k} sentences per language to study the results under different data sizes. 
%The results with {\it 200k} and {\it 1000k} sentences are shown in Sections~\ref{subsubsection:small} and~\ref{subsubsection:big}, respectively.  

Surprisingly, when pre-trained on small pretraining data (200k sentences per language), BERT didn't show its extraordinary cross-lingual ability as shown in Figure~\ref{fig:3_1} and \ref{fig:3_2}. For example, GloVe and Word2Vec achieved stronger cross-lingual alignment than BERT in terms of MRR score on word retrieval task on every language paired with English. And although BERT achieved better accuracies on XNLI zero-shot transfer on several languages, the margins were very small, and the overall performances were not better than GloVe and Word2Vec.  

This finding provides a further discussion of the literature. Work by ~\citet{Karth:20} has found that depth and the total number of network parameters were two decisive architecture elements dominating the cross-lingual ability of BERT, also supported by experiments on XNLI. 
When the number of attention heads and the number of total parameters were fixed, decreasing model depth degenerated cross-lingual transfer performance. On the other hand, when the number of attention heads and depth were fixed, decreasing the number of network parameters degenerated performance, either. 
It seems that the expressiveness or capacity of models is crucial to building up cross-lingual ability. 

However, is it really the case that the bigger, the better? 
From results in this experiment, the capacity of BERT is definitely much bigger than GloVe and Word2Vec, but in the case of pretraining on the limited size of data, BERT didn't achieve superior performance as expected, suggesting that the relation of model capacity and cross-lingual ability may not be monotonic and the size of pretraining data also comes into play. 

\subsection{Big Pretraining Data}
\label{subsubsection:big}

When pre-trained on big pretraining data (1000k sentences per language), there was a dramatic turn as shown in Figure~\ref{fig:3_3} and~\ref{fig:3_4}. BERT achieved an overwhelmingly higher MRR score than other embeddings on every XX-En language pairs, showing that it did a much better job in aligning semantically similar words from different languages. 

Testing results on XNLI were also consistent with word retrieval task, BERT reached higher accuracies than GloVe and Word2Vec, demonstrating that it had the better cross-lingual ability.  

It was noticeable that the increase in pretraining data size largely improved the cross-lingual alignment and transferability of BERT, while it was not the same case for GloVe and BERT. And the bounding performance of Google BERT, which is the pretrained parameters released by Google, shows that there is still room for improvement if given even more pretraining data.

Besides the effect of amount of data, in the next subsection, we further studied other key components making BERT capable of learning a good cross-lingual representation space.


\subsection{Breaking Down Long Dependency}
We noticed that the typical co-occurrence window size of non-contextualized embeddings, like GloVe and Word2Vec,  are often limited to 5$\sim$30 tokens, but BERT could attend to hundreds of tokens, which means that BERT could learn from longer dependency and richer co-occurrence statistics. So we experimented with a smaller window size to find out if longer dependency is also necessary for learning cross-lingual structures.    
We directly sliced sentences in original pretraining data into smaller segments, limiting input length to 20 tokens for each example. And then we evaluated embeddings pretrained on these segments for cross-lingual ability\footnote{Limiting the number of tokens attended by attention heads may not work because the information from far tokens could still flow through layers and be collected at deeper layers.}.   


Results are shown as figure~\ref{fig:3_5}. In the case of big pretraining data, pretraining BERT with shortened inputs drastically hurt the cross-lingual ability of BERT, indicated by lower MRR score on word retrieval task compared to BERT pre-trained on normal-lengthed data. It should be noticed that the total number of tokens in pretraining data stayed unchanged.

However, in the case of small pretraining data, pretraining BERT with shortened inputs yielded to better cross-lingual alignment on several languages, suggesting that breaking down long dependency helps BERT to learn better cross-lingual alignment when only limited data is available.  

In Figure~\ref{fig:3_6},  it is shown that when there were no long dependencies to learn, the benefit of increasing the datasize became minor. 
The results on XNLI also show that breaking down long dependency was more harmful when there were more pretraining data.   


We further checked the case of Word2Vec, varyring window size to 128 and 256 on small pretraining data. The alignment evaluation via MRR is shown in Figure~\ref{fig:3_7}. On most of the languages, increasing window size to 128 improved cross-lingual alignment on Word2Vec embeddings. However, increasing window size to 256 was not as beneficial, suggesting there may be a bottleneck from model capacity.

Considering the above observations, we hypothesized that cross-lingual alignment or cross-lingual transferability of BERT are learned not only from local co-occurrence relations but also from co-occurrence relations of global scope, with a larger amount of data and model capacity required.

\subsection{Word Retrieval Part-of-speech Analysis}
At last, to gain insight into where alignment happens and which type of tokens are aligned best in our pretrained BERT (1000k), we analyzed the MRR score by part-of-speech tag obtained from the OntoNotes Release 5.0~\footnote{https://catalog.ldc.upenn.edu/LDC2013T19}dataset. We simply associated each token in m-BERT vocabulary with its most common part-of-speech label from OntoNotes annotations and calculated MRR for each class of part-of-speech tag. For simple comparison, we further grouped all the part-of-speech tags into closed-class and open-class two classes, as shown in table~\ref{tab:mrr_by_pos}, where fixed sets of words serving grammatical functions fall into closed-class and lexical words (e.g. noun, verb, adjective and adverb) fall into open-class. Different from \citet{Cao2020Multilingual}'s work, we showed that our BERT has higher alignment score for open-class versus closed-class categories. And among open-class of part-of-speech tags, adjectives are better aligned, on top of nouns, adverbs and verbs.        


\begin{figure*}[t!]
\centering
\begin{subfigure}[b]{\columnwidth}
\includegraphics[width=\linewidth]{sections/figs/mrr_small.pdf}
 \subcaption{ Except for Google Bert, embeddings were pre-trained on 200k sentences per language.}
 \label{fig:3_1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{\columnwidth}
\centering 
\includegraphics[width=\linewidth]{sections/figs/mrr_big.pdf}
 \subcaption{Except for Google Bert, embeddings were pre-trained on 1000k sentences per language..}
 \label{fig:3_3}
\end{subfigure}
\caption{Evaluating alignment with Word Retrieval, compared between different representation models. For reference, Google BERT is the m-BERT pre-trained by Google.}
\end{figure*}

\begin{figure*}[t!]
\centering 
\begin{subfigure}[b]{\columnwidth}
\includegraphics[width=\linewidth]{sections/figs/XNLI_small.pdf}
 \subcaption{Pre-trained on 200k sentence per language}
 \label{fig:3_2}
\end{subfigure}
\hfill
\begin{subfigure}[b]{\columnwidth}
\centering 
\includegraphics[width=\linewidth]{sections/figs/XNLI_big.pdf}
 \subcaption{Pre-trained on 1000k sentence per language}
 \label{fig:3_4}
\end{subfigure}
\caption{Performance comparison on XNLI zero-shot cross-lingual transfer task}
\end{figure*}

\begin{figure*}[t!]
\begin{subfigure}{\columnwidth}
  \includegraphics[clip,width=\linewidth]{sections/figs/windowsize_200.pdf}%
\end{subfigure}
\hfill
\begin{subfigure}{\columnwidth}
  \includegraphics[clip,width=\linewidth]{sections/figs/windowsize_1000.pdf}%
\end{subfigure}
\caption{The Effect of Window Size}
\label{fig:3_5}
\end{figure*}


\begin{figure*}[t!]
\begin{subfigure}[b]{\columnwidth}
  \includegraphics[clip,width=\columnwidth]{sections/figs/windowsize_xnli_all.pdf}
  \subcaption{When limiting context window, the effect of pretraining datasize is less significant on XNLI transfer performance}
\end{subfigure}

\begin{subfigure}[b]{\columnwidth}
  \includegraphics[clip,width=\linewidth]{sections/figs/windowsize_xnli_decrease_per.pdf}
  \subcaption{Performance drop on XNLI due to limiting context window size (original 512$\rightarrow$20) is shown in percentage. It is shown that the performance decrease of BERT pre-trained on small data is less than big data and even negative on some languages, which means there is an increase in transfer}
\end{subfigure}
\caption{The Effect of Window Size}
\label{fig:3_6}
\end{figure*}

\begin{figure}[t!]
\centering 
\includegraphics[width=\linewidth]{sections/figs/Word2Vec (1).pdf}
 \caption{The Effect of Window Size on Word2Vec}
 \label{fig:3_7}
 \vspace{-0.25cm}
\end{figure}
\input{sections/tables/mrr_by_label}

==> sections/relate.tex <==
\section{Related Work}
\textbf{Multilingual BERT.} BERT~\citep{devlin:19} is a Transformer-based~\citep{vaswani:17} large pre-trained language model that has been widely applied in numerous NLP tasks, showing great potentials in transfer learning. And m-BERT, which is pre-trained on Wikipedia text from 104 languages without cross-lingual objective or parallel data, serves as a good cross-lingual representation model that generalizes well across languages for a variety of downstream tasks~\cite{wu:19, hsu-etal:19, pires:19}. There are a line of works studying the key components contributing to the cross-lingual ability of m-BERT~\citep{Karth:20, tran:20, Cao:20, singh:19}, sometimes coming with inconsistent observations, showing that our understandings about it are still in the early stages.\\

\noindent\textbf{Cross-lingual Word Embedding.} The goal of cross-lingual word embedding is to learn embeddings in a shared vector space for two or more languages. A line of works assumes that monolingual word embeddings share similar structures across different languages and try to impose post-hoc alignment through a mapping~\citep{mikolov:13, Smith:17, joulin:18, Lample:18, artetxe:18, Zhou:19}. Another line of works considers joint training, which optimizes monolingual objective with or without cross-lingual constraints when training word embeddings~\citep{luong:15,gouws:15,Ammar:16,duong:16,lample:18b}. Cross-lingual word embedding methods above were initially proposed for non-contextualized embedding such as GloVe~\citep{pennington:14} and Word2Vec~\citep{mikolov:13w2v}, and later adapted to contextualized word representation~\citep{schuster:19, aldarmaki-diab:19}. Recently, token representations from m-BERT also serve a similar role as cross-lingual word embedding in many works.           
